In Perfect Shape: Certifiably Optimal 3D Shape Reconstruction from 2D Landmarks

We study the problem of 3D shape reconstruction from 2D landmarks extracted in a single image. We adopt the 3D deformable shape model and formulate the reconstruction as a joint optimization of the camera pose and the linear shape parameters. Our first contribution is to apply Lasserre's hierarchy of convex Sums-of-Squares (SOS) relaxations to solve the shape reconstruction problem and show that the SOS relaxation of minimum order 2 empirically solves the original non-convex problem exactly. Our second contribution is to exploit the structure of the polynomial in the objective function and find a reduced set of basis monomials for the SOS relaxation that significantly decreases the size of the resulting semidefinite program (SDP) without compromising its accuracy. These two contributions, to the best of our knowledge, lead to the first certifiably optimal solver for 3D shape reconstruction, that we name Shape*. Our third contribution is to add an outlier rejection layer to Shape* using a truncated least squares (TLS) robust cost function and leveraging graduated non-convexity to solve TLS without initialization. The result is a robust reconstruction algorithm, named Shape#, that tolerates a large amount of outlier measurements. We evaluate the performance of Shape* and Shape# in both simulated and real experiments, showing that Shape* outperforms local optimization and previous convex relaxation techniques, while Shape# achieves state-of-the-art performance and is robust against 70% outliers in the FG3DCar dataset.

==> fig-FG3DCar_qualitative.tex <==
%!TEX root = main.tex

\newcommand{\mpwthree}{3cm}
\newcommand{\myhspace}{\hspace{-3.5mm}}

\begin{figure*}[h]
	\begin{center}
	\begin{minipage}{\textwidth}
	\begin{tabular}{cccccc}%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\myhspace \alternrobust & \myhspace \convexrobust & \myhspace \SOSGNCTLS & \myhspace \alternrobust & \myhspace \convexrobust & \myhspace \SOSGNCTLS \\
		\hspace{-5mm}
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_00_altern_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_00_convex+refine_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_00_SOS_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage} 
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_10_altern_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_10_convex+refine_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage}
		&  \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_10_SOS_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage} \\
		\multicolumn{3}{c}{(a) Chevrolet Colorado LS $0\%$ outliers. } & \multicolumn{3}{c}{(d) BMW 5-Series $0\%$ outliers.} \\
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\hspace{-5mm}
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_40_altern+robust_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_40_convex+robust+refine_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_40_GNC-TLS_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_40_altern+robust_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_40_convex+robust+refine_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_40_GNC-TLS_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage} \\
		\multicolumn{3}{c}{(b) Chevrolet Colorado LS $40\%$ outliers.} & \multicolumn{3}{c}{(e) BMW 5-Series $40\%$ outliers.} \\
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\hspace{-5mm}
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_70_altern+robust_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_70_convex+robust+refine_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{056_70_GNC-TLS_Chevrolet_Colorado-LS_2004_06.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_70_altern+robust_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_70_convex+robust+refine_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage}
		& \myhspace
			\begin{minipage}{\mpwthree}%
			\centering%
			\includegraphics[width=\columnwidth]{035_70_GNC-TLS_BMW_5-Series_2011_05.pdf} \\
			\vspace{1mm}
			\end{minipage} \\
		\multicolumn{3}{c}{(c) Chevrolet Colorado LS $70\%$ outliers.} & \multicolumn{3}{c}{(f) BMW 5-Series $70\%$ outliers.} \\
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


		\end{tabular}
	\end{minipage}
	\vspace{-2mm} 
	\caption{Selected qualitative results on the \FGCar dataset~\cite{Lin14eccv-modelFitting} under $0\%$, $40\%$ and $70\%$ outlier rates using \alternrobust~\cite{Zhou17pami-shapeEstimationConvex}, \convexrobust~\cite{Zhou17pami-shapeEstimationConvex}, and \namerobust. (a)-(c): results on the Chevrolet Colorado LS; (d)-(f): results on the BMW 5-Series. Green: inliers. Red: outliers. Circle: 3D landmark. Square: 2D landmark. [Best viewed electronically.]
	\label{fig:FG3DCar_qualitative}}
	\vspace{-7.5mm} 
	\end{center}
\end{figure*}
